Semantic Linking Maps for Active Visual Object Search

We aim for mobile robots to function in a variety of common human environments. Such robots need to be able to reason about the locations of previously unseen target objects. Landmark objects can help this reasoning by narrowing down the search space significantly. More specifically, we can exploit background knowledge about common spatial relations between landmark and target objects. For example, seeing a table and knowing that cups can often be found on tables aids the discovery of a cup. Such correlations can be expressed as distributions over possible pairing relationships of objects. In this paper, we propose an active visual object search strategy method through our introduction of the Semantic Linking Maps (SLiM) model. SLiM simultaneously maintains the belief over a target object's location as well as landmark objects' locations, while accounting for probabilistic inter-object spatial relations. Based on SLiM, we describe a hybrid search strategy that selects the next best view pose for searching for the target object based on the maintained belief. We demonstrate the efficiency of our SLiM-based search strategy through comparative experiments in simulated environments. We further demonstrate the real-world applicability of SLiM-based search in scenarios with a Fetch mobile manipulation robot.

==> NOTES.tex <==
\subsection{Robotic retrieval of objects / object search includes}
\begin{itemize}
\item \textbf{local search} of objects in clutter in an interactive/active manner
\item search for objects in \textbf{semantic places} based on correlations/contextual relations between object and places. Then this divides into search in unfamiliar and familiar environments. For unfamiliar, common sense knowledge is being used. For familiar environment, (where is waldo? work, any more works?). Highlight papers that make sure of scene graph for object search (prior assisted object search paper, and papers that cite it), point out why that is beneficial. Our paper takes similar approach to the prior-assisted paper, but our difference is such and such(instead assuming known scene graph of the environment, we infer that from the past observations). Highly related paper is indirect object search paper, but they do not monitor the changes in the scene, and update the belief of where object is.
\end{itemize}

\subsection{Semantic mapping for object search.}
\begin{itemize}
    \item semantic mapping works; not directly targeted at object search, do not take temporal factor into account.
    \item semantic mapping that model the object dynamics; (recent arxiv paper, and the papers it cites); not sure whether the representation is readily usable for motion planning or controller systems.
\end{itemize}


Notes:
\begin{itemize}
    \item Also cite \emph{Act to See and See to Act} by Li, Hsu and Lee
    \item Paper by Kunze et al. \cite{kunze2014using} is our strongest competitor! They use qualitative spatial relations across multiple objects to infer most likely object locations. They have a method of converting the spatial relations into Gaussian distributions they can sample locations from. Things they don't have but we do:
    \begin{itemize}
        \item Pose estimation
        \item A perception control loop for active perception. They pre-compute possible voxels the objects could be in, select a robot location from a fixed set of poses and then try to find the best view cone. I think our approach is more robust because it uses continuous spaces and can also adapt itself to changes in perception.
        \item They seem to need to make a distinction between static and dynamic objects. We don't, which makes us more flexible.
    \end{itemize}
    \item Paper by Xiao et al. \cite{xiao2019online} is seemingly the most recent work in this field. They do interactive perception to find a potentially occluded object on a table top, in the process of which they estimate the poses of objects both to rate object occlusions and to be able to manipulate them. They develop sample generators which are able to instantiate simulation scenarios based on assumptions made about unobserved variables. These simulation scenarios are used to back a POMDP solver called POMCP. The overall problem is formulated as a POMDP and the authors show that their system outperforms other methods significantly in their experiments.
    Contrasting their work to ours is not that difficult. We are focused on a much larger operational domain and aim for a reactive approach, over an optimal solution. They don't employ any inter-object relationships, probably making their method hard to apply to a large environment. 
    It is important to us to integrate the real-time perception updates into our motions and avoid using generation methods like the ones by Xiao et al. by simply resampling our particles. This way we can actually also deal with occluded objects, however we do not need to classify them, or estimate their poses. Granted, interactive perception would be difficult with our approach. 
    \item Paper by Eidenberger and Scharinger \cite{Eidenberger2010IROS} describes Gaussian pose mixtures similarly to how we do it and describes an \textit{incremental} observation behavior, which is very similar to what our controller exhibits in case of occlusions.
    \item Paper by Potthast and Sukhatme \cite{Potthast2016IROS} deals with trajectory optimization for observation. Its set in the realm of quadrotors, but some of the constraints are similar. No Gaussians though.
    \item Paper by Kaelbling and Lonzano-Perez \cite{kaelbling2012unifying} tries to do a similar thing to us, but I think they're too focused on modelling observed and unobserved space, rather than object locations.
    \item Paper by Wong, Kaelbling and Lonzano-Perez \cite{wong2013manipulation} tackles the problem of perceiving potentially occluded objects in containers. They make use of the notion of object co-occurrence and provide some citations for the notion's usefulness. They record object occurrences and co-occurrences to infer the object types which are likely to be contained in a container. They also consider geometric feasibility by keeping track of the unobserved space in a container and filling it with likely, remaining objects. I think some parts of this work are related to what we are doing. Though they don't do it in a symbolic fashion, they do use object occurrances and co-occurrances to inform their search. Their search has a comparatively flat hierarchy, due to them only considering the \emph{in} and \emph{nextTo} relations. An interesting difference between this work and ours is the model of observed space. While they do it explicitly through an oct-tree, we do it implicitly by re-sampling the particles in our perception system. I think that is a distinction we should think about stating explicitly.
    \item Paper by Nie, Wong and Kaelbling \cite{nie2016searching} concerns itself with finding objects in cluttered containers. It has an observation model, but uses discrete view points, coined \emph{view windows}, and a cost function which trades off moving to another view point against picking up an object to potentially reveal an occluded target object. For our view control this is probably not of much use, but I think an analogy can be drawn between our spawned particles in containers and their sample generation.
    \item The article by Loncomilla et al. \cite{loncomilla2018bayesian} focuses on providing a Bayesian methodology for informed robotic object search. In their method, Loncomilla et al. aim to support arbitrary inter-object relations. They make use of so called relation masks which are able to describe sharp and soft possibility spaces and can be layered on top of each other to create a final positional distribution. They evaluate their system in simulations and real experiments, while using different search strategies.
    As far as I understand it, the approach is somewhat similar to ours, but then also not really. The usage of object relations and probabilistics is similar, but our environment models are deeper. On the execution side they use more planning than we do, and they can actually re-plan during their execution, but that seems to only occur in fixed intervals or when a previous goal is reached. This makes our approach more reactive. They also discretize their distributions to come up with potential object locations and camera view poses. One important take-away from their related work section though: We are doing informed, indirect object search.
    \item The search system based on the CORTEX architecture by Gutiérrez, Manso, N{\'u}{\~n}ez and Bustos \cite{gutierrez2018planning} is similar to what we are doing. \adrian{EDIT: Upon re-reading it, it's actually not. It focuses entirely on the building up of a semantic prior. I'll leave the previous notes here, but it actually doesn't relate} Differences:
    \begin{enumerate}
        \item The robot needs to map out its environment beforehand. We technically don't have to do that, because of the common sense knowledge, but practically we still do it.
        \item Their overall process is very different. They do a kind of mental imagery when asked to look for an object. They go through the images they've recorded during the exploration, classify the objects on them and compute label vectors for the individual tables. During search they then approach the table coincides most with the desired label. They compare their approach to a random table approach and a traveling salesman approach of the tables. Their simple table selection outperforms the other two algorithms which strengthens our argument. From my reading, they don't use a distance metric as a factor in their table approach. 
    \end{enumerate}
    \item Temporal Persistence Modelling by Toris and Chernova \cite{toris2017temporal} is very focused on the temporal persistence model (TMP) and less on practical application. Their model can infer at which semantic location an object is going to be at a point in time. This inference is probabilistic and based on sparse, prior observations. They do not seem to give a geometric interpretation for the object locations, so I'd argue that it'd be hard to use their method for pose estimation. Overall though the method is far more interested in predicting the locations over time, than in space. I think in that way we are actually not in any competition with them. I'm not sure about the mathematical overlap.
    \item Efficient Object Search With Belief Road Map Using Mobile Robot by Wang et al.\cite{wang2018efficient} is similar to the 2013 paper by Aydemir et al. \cite{aydemir2013active}. They try to find objects on a room level but use a POMDP as planning mechanism. They have a lot of analyses going on and admittedly I did not get all of it from my first read. Different from Aydemir, they have a previously mapped out space. I think this paper warrants a more in-depth look, but my first impression is that there's not a lot there from our perspective.  
\end{itemize}

==> NOTES_EXP.tex <==
To support our claims of our contributions, we need to design experiments around our claims. For following claims, experiments that we need:
\begin{itemize}
    \item Claim: accounting for object spatial dependencies via the factor graph is beneficial; Baseline: w/o modeling object dependencies at the semantic level, simply summarizing object position distribution, and use that for search; v.s. our method. Here are the failure cases to highlight (in terms of Figures Qualitative examples):
    \begin{itemize}
        \item supporter case (4. and 5. in Adrian's list): objects wrongly fitted to structure (with or without false positive detection fired) that is within the spread of its position distribution, because it does not first actively look for where the table is and shrink the search space of object location accordingly based on the object dependencies. While our method is robust to these kind of failure cases.
        \item container case (5. in Adrian's list): in case of occlusion due to containers, the probability of object location on other supporting tables will grow higher than hypothesis in current view, which motivates the robot to move to other places for object search. While our method localizes the container, and hypothesize that the object could be inside of the container, that motivates the robot to look into the container. \todo{I think 5. is not an appropriate test. It is only defined as occlusion. I'm writing the setup down in 3), but think we should talk about this. -Adrian}
        \item neighbor case (6. in Adrian's list): looking for coke, and baseline ignores the fact that sprite is highly correlated as a neighbor of coke. During search, sprite is detected, hypothesis of coke around sprite location should become higher than other locations with clutter (e.g. tools clutter) on the table.
        \item basically observations of supporter and/or container and/or neighboring object will increase the probability distribution differently than the pure metric (non-semantic) approach
        \item failed to find object at predicted location (2. on Adrian's list): Show, by 1) qualitative highlights of recovery behavior with updated scene graph and robot looking at new promising location pictures 2) recovery rate among all the experiments.
    \end{itemize}
    \item Claim: ablation study on different factors in the factor graph for representing GOP. Qualitative examples in figures.
    \begin{itemize}
        \item only common sense knowledge: show target object GMM spread uniformly on all table
        \item common sense knowledge + long term memory (3. in Adrian's list): show target object GMM spread unevenly on all table based on past observation
        \item common sense knowledge + long term memory + short term memory: show target object GMM changes based on short term observation: 1) probability raises around found target object neighbor; 2) probability drops where target object is not found.
    \end{itemize}
    \item Claim: Control is great!
    \begin{itemize}
        \item Show \textit{Change of mind} with qualitative examples (7. on Adrian's list)
        \item 
    \end{itemize}
\end{itemize}

==> NOTES_INTRO.tex <==
\subsection{guideline from our discussion}
\begin{itemize}
    \item general motivation for object search. Introduce generalized object permanence $\rightarrow$ connection to object search. How we are modeling gop, with what factors. active perception. what experiments we show.
    \item brief peek into the related work:
    \begin{itemize}
        \item object search in local workspace: examples (Jue Kun Li, 2016, Yuchen Xiao ICRA 2019, Larson Wang, etc)
    broad statement: hard to scale to large scale, perception always simplified. Not modeling the semantics of the scene structure and reasoning about inter-object relations for object search, mainly geometrically reasoning on 3D occupancy.
        \item object search in large workspace: examples (Aydemir, Chaoqun Wang ICRA 2018, etc)
    broad statement: they search for the object at coarse level, once they enter the room that the object can be in, they basically sweep the volume to look for the object without too much strategy.
    \end{itemize}
    
    \item three most related work
    \begin{itemize}
        \item Nick Hawes et al. "Using Qualitative Spatial Relations for Indirect Object Search": also use object spatial relation to direct the object search process. talk from the active perception action perspective (Adrian's expertise!)
        \begin{itemize}
            \item they assume all target objects are going to be on detected supporting planes, instead of generalizing over inter-object relations, such objects placed on different tables
            \item their spatial relation is limited to 2D, restricting the expression power of the scene structure
        \end{itemize}
        
        \item similar to (b): Topological spatial relations for active visual search. The search strategy is the same with ours in that they follow the hierarchical scene graph structure to search for target object. E.g. book in box on table, then it looks for table, then box, then book. The contrast to our work is:
        \begin{itemize}
            \item they assume given true scene graph (or in other world object spatial relations), but we don't assume given and instead maintaining a belief over it
        \end{itemize}
        
        \item  Oliver Brock IROS 2014: also use factor graph to model object spatial relation, and our reasoning module is inspired by that. Two main contrasts: 
        \begin{itemize}
            \item we realized it on real robot, where we need to deal with practical perception and action problems. 
            \item they assume perfect perception such that only object relations involving target object is unknown, we are problematically modeling the perception problem where we maintain a belief of all object relations
        \end{itemize}
    \end{itemize}
\end{itemize}

==> SEPTEMBER_EXP.tex <==
\subsection{Evaluating Object Detection and Pose Estimation}
To evaluate the benefits of using semantic spatial object relations for object detection and pose estimation, we devised two experimental setups.
\begin{enumerate}
    \item Our factor graph reflects that our searched objects are supported by other objects on a room-scale. The search behavior is tasked with finding the same objects multiple times, each time starting at the same location. However, for each run the supporting objects change their positions by up to a meter.
    Our approach is compared to a baseline which is using a purely metric representation for potential object locations. The goal objects' metric locations have a much greater variance due to the variance in the supporting objects' locations. 
    \todo{Isn't this a very forced scenario? Which household supporter actually changes positions this much? Maybe chairs? Or chopping boards with knives on them?}
    We expect our approach to be more efficient in locating objects in this scenario. The more confined search space which results from the semantic object relations, will give our approach an edge over the baseline.
    Further, we expect our approach to outperform the baseline especially in cases where the searched object is occluded. Without the constraint of the semantic relationship, the particles used for the pose estimation will disburse, causing the focus of the system to needlessly shift to other areas.
    Lastly, we expect our approach to produce less false-positive recognitions, since false positives are unlikely to satisfy the semantic constraints.
    \item The previous setup seeks to examine the benefits of having a hierarchical structure for object locations. The goal of this second setup is to evaluate the benefits of the neighboring relationships. 
    In a semi-cluttered tabletop scenario, there are multiple possible occluded areas for the searched object to be located in. Close to some of these is another object which is often in the neighborhood of the searched object. This relationship guides the search of our approach.
    We expect our approach to outperform a purely metric baseline, since it will do an unguided search of the occluded areas.\todo{Maybe this not a good baseline. Instead supporting-, but no neighboring relationships?}
    \item \todo{The container case. Thought: It might actually not belong as its extra thing, but rather with 2), Because both talk about how the semantics help in dealing with occlusions.}
\end{enumerate}

\subsection{Evaluating Adaptability}
The previous section focused on proposing methods for evaluating the benefit of combining semantic inter-object relations and metric observations. In this section we propose experiments which will show the factor graph's ability to incorporate newly made observations.
\begin{enumerate}
    \item TODO
\end{enumerate}

==> discussion.tex <==
\section{Discussion}
The accuracy of the object detector greatly influences the overall performance of search behaviors. State-of-art deep learning methods, such as Faster-RCNN that we used in the experiments, are susceptible to the lighting conditions. The reflection on objects due to strong lights can cause many false negatives, and restrain the performance. However, our method has the advantage of using belief samples, which can guide robots to explore some specific areas more diligently, and lead to active or interactive search actions, such as removing occlusions.

% Though the simple metric for picking a Gaussian component to investigate has proven itself to be useful, it also leads to an over-investigation of potential locations in small spaces. To avoid this, we propose extending the rating of Gaussian components to include an estimated perceptual effort. This effort would take the degree of separation between the target- and supporting object in the scene graph into account, as well as a baseline effort needed to perceive different types of objects. This notion of effort could be used in one of two ways to accommodate the different execution costs between active and interactive perception. Either the effort could be seen as an upper bound on a budget of system cycles to be spent on the investigation of a particular Gaussian component. As long as the budget is not depleted, further action to investigate the component is being taken.
% The second way would be to not only consider the degree of separation, but also the type of separation. If an object is inside a container, this might imply a costly manipulation action opening the container. While the latter method is closer to the current approach, it requires either more information about the objects' states, or costs for observing some relations on an object need to be learnt as well.

%\rephrase{is this addressed?}{Adrian}\zhen{discussion on how we can make decisions (or how we are making the decisions, it is ok even if it is simple as long as we can make an argument that the existing works are also limited in making a good decision on it, and we leave that to future work) on whether using manipulation action or mobile navigation to explore an occluded region. My understanding is that works that use POMDP formulations can make decisions on that by maximizing the reward, but they will need good knowledge/heuristic of the 3D occupancy of the unobserved area, and good heuristic of the "information gain" resulting from the manipulation action v.s. mobile navigation, which in itself is hard to model for general cases.}

%Note that enabling the robot to autonomously explore and semantically map the environment for collecting past observations is not the focus of this paper, and that it is worth investigating as part of future works.

==> implementation.tex <==
\section{Implementation}
\subsection{Observation Controller and Search Behavior}
The observation controller is implemented using the \textit{giskardpy}\footnote{\url{https://github.com/SemRoCo/giskardpy}} library, which is the current implementation of the motion control framework proposed in \cite{fang16simcontrol}.
For collision checking, we use the \textit{Bullet}\footnote{\url{https://github.com/bulletphysics/bullet3}} physics engine, an open-source collision-checking and physics simulation library.
Both the controller and the behavior are implemented as components of the \textit{GeBSyAS}\footnote{\url{https://github.com/aroefer/gebsyas}} framework, which seeks to unify geometrical data and symbolic predicates in one cohesive model. 
The giskardpy-framework uses a gradient descent method for generating control signals. The kinematics of the base of the fetch robot make it difficult to define control terms for sideways motion, since the base can only move forwards and backwards and turn around its vertical axis. These kinematics caused very slow motions when escaping occluded viewpoints. To prevent this, we employ an external navigation framework in these scenarios. 

==> methods.tex <==
\section{Methods}
Our method consists of three parts: (1) probabilistic modeling of inter-object semantic spatial relations $R_{ij}$, (2) maintaining the belief over object locations $P(O_T|x_{0:T, z_{0:T}})$, and (3) a search strategy that considers view pose selection.

To perform object search, we first model the probabilistic distribution of inter-object semantic spatial relations between all object pairs in the environment based on common sense knowledge. Then this relation is taken into account as we maintain the belief over object locations. Upon a request to search for a target object, we sample and select the best next view pose for the robot to navigate to based on the belief \rephrase{over object locations.}{This sounds unclear. Is it the belief over the target object's location, or over all object locations?} Then robot alternates between the belief update of objects' locations and view pose selection, until the target object is found or the maximum search time is reached.

\input{probabilistic_relation.tex}
\input{object_belief.tex}
\input{view_pose_selection.tex}

==> questions.tex <==
\subsection{Questions}
Questions to be answered while writing up this paper:
\begin{itemize}
\item how do people plan for object search? mainly among the works that uses semantic locations for object search, instead of the local search
\item how do people accumulate multiple observations of an environment for semantic mapping, that can be potentially useful for object search? how do they deal with dynamic objects and how are we dealing with them?
\item how does our method compare to life-long learning works?
\end{itemize}

==> scenarios.tex <==
\subsection{Scenarios}
There are several typical scenarios that we are dealing with during robotic retrieval processes. These scenarios can be categorized based on 1) how the target object location has changed since the last visit, and 2) what has been observed.

Based on how the target object location has changed since the last visit, there are the following cases:
\begin{itemize}
\item The object stays at the same metric location
\item The object stays at the same semantic location with changed metric location. For example, a milk bottle is still placed on the same table, but not in the exact same spot.
\item The object changes its semantic location. For example, a milk bottle is moved from the table into the fridge/cabinet. Is it reasonable to assume that objects are more likely to transit to nearby (metric-wise) semantic locations instead of further ones within a short period of time? This would make sense, for example, the milk bottle has been observed on the counter by the side of fridge A recently, then the milk bottle is more likely to be stored in fridge A after that than in fridge B that is far away from the counter maybe in a different room. (This indicates that we want to model the dynamics of objects over time, e.g., fridge and cabinets are static, many tables like office tables are going to be somewhat static, many tabletop objects are going to be dynamic, and a coffee table will be quasi-static, these can either be learned or hand-coded, or learned starting from some prior.)
\item The object stays at either the same metric location relative to its semantic location or stays at the same semantic location, but the semantic location itself has changed location. For example, cereal was observed to be placed in a box, and cereal stays in the box, but the box has been moved to a different location.
\end{itemize}

Based on what has been observed by the robot, there are the following cases:
\begin{itemize}
\item The robot has observed the target object recently
\item The robot has observed an object contextually related to the target object recently. For example, knowing that cereal is contextually related to milk bottles, it is reasonable to hypothesize that the milk bottle can be somewhere around where the cereal was observed recently.
\end{itemize}

As contexts for the evaluation of our approach, we choose two larger tasks for the robot to complete: Making preparations for a movie-night, and putting away a few groceries. The movie-night task is largely a retrieval task, in which the robot needs to procure a set of items from different locations in a mapped environment, and deliver them to a known location. The probable object locations are inferred by the reasoning module.\todo{Formulation needs a touch-up}
The grocery task is the inversion of the movie-night task. The robot needs to put away a set of groceries, for which the locations are inferred by the reasoning module. This task is suited especially well for evaluating how well the graphical model performs at learning the unique structure of an environment.

\textbf{INTERNAL}

In terms of practical implementation, we have agreed on the 2nd floor student lounge being the goal location for both tasks. For the retrieval task there is a single caveat: All objects need to be outside of the lounge. Otherwise the robot will grab and take them for a little walk, while it moves on to fetching other things.

==> scope.tex <==
\section{Scope}
The robot gathers \textbf{multiple} objects from the environment for a task (e.g., to support further human activities), which involves \textbf{actively searching} for objects, \textbf{manipulating} them and \textbf{explore occluded} regions through mobile navigation and manipulation actions such as container opening. 

\begin{itemize}
    \item Multiple object retrieval (have a box at the base for collection)
    \item Manipulation (pick and drop, pick up container lid)
    \item Put things away (one thing at a time, drop into container), really a subset of search routine
\end{itemize}
